Scaling Laws For Dense Retrieval

Scaling up neural models has yielded significant advancements in a wide array of tasks, particularly in language generation. Previous studies have found that the performance of neural models frequently adheres to predictable scaling laws, correlated with factors such as training set size and model size. This insight is invaluable, especially as large-scale experiments grow increasingly resource-intensive. Yet, such scaling law has not been fully explored in dense retrieval due to the discrete nature of retrieval metrics and complex relationships between training data and model sizes in retrieval tasks. In this study, we investigate whether the performance of dense retrieval models follows the scaling law as other neural models. We propose to use contrastive log-likelihood as the evaluation metric and conduct extensive experiments with dense retrieval models implemented with different numbers of parameters and trained with different amounts of annotated data. Results indicate that, under our settings, the performance of dense retrieval models follows a precise power-law scaling related to the model size and the number of annotations. Additionally, we examine scaling with prevalent data augmentation methods to assess the impact of annotation quality, and apply the scaling law to find the best resource allocation strategy under a budget constraint. We believe that these insights will significantly contribute to understanding the scaling effect of dense retrieval models and offer meaningful guidance for future research endeavors.

==> chapters/2_relatedwork.tex <==
\section{Related Works}
In this section, we recap related work in dense retrieval and domain adaptation.
\subsection{Dense Retrieval}
Dense retrieval models encode the query and the document into dense vectors and use nearest neighbor search to retrieve documents. Earlier works focused on exploring training strategies for DR models, such as hard negative mining techniques~\cite{xiong2020approximateANCE,zhan2021optimizingADORE,zhan2021optimizingHard} and knowledge distillation from a strong cross-encoder~\cite{qu2020rocketqa,hofstatter2021efficiently,lin-etal-2021-batch}. Recent works investigate how to perform retrieval-oriented second-stage pre-training on large language models~\cite{gao2021condenser,gao2021unsupervised,izacard2022unsupervised,liu2022retromae,maxinyu}.

\subsection{Zero-Shot Dense Retrieval}
Thakur et al.~\cite{thakur2021beir} collected the BEIR benchmark, which consists of diverse retrieval tasks from different domains. They evaluated dense retrieval models and challenged the generalization ability of DR models. Many later works follow this Zero-shot DR setting, where the DR model is trained using a diverse and richly supervised retrieval dataset and then evaluated on the out-of-domain search corpus, which is usually accessible during training. Furthermore, recent research have shown that there is a certain correlation between distribution shifts and zero-shot performance.

\subsection{Domain Adaptation}
Previous work on domain adaptation for IR can be roughly divided into three categories. The first category is the traditional Unsupervised domain adaptation (UDA) methods, such as MoDIR~\cite{xin-etal-2022-modir}, which encourages the DR models to learn a domain invariant representation space that facilitates the generalization from source to target through momentum and adversarial learning.
The second category mainly focuses on query generation techniques. These methods generate additional auxiliary training data on the target domain with the help of a well-tuned generation model~\cite{ma-etal-2021-qgen}, or further employs a powerful cross-encoder to generate pseudo-labels for distillation~\cite{wang-etal-2022-gpl}.
The third category is retrieval-oriented pre-training. These methods employ pre-training tasks specially designed to improve the retrieval performance of DR models. 
TSDAE~\cite{wang-etal-2021-tsdae-using} leverages an additional denoising auto-encoder to pre-train the DR model with 60\% random tokens deleted in the input document.
Condenser~\cite{gao2021condenser} and coCondenser~\cite{gao2021unsupervised} enhance the representation of [CLS] token and introduces the Sequence Contrastive Learning (SCL) task for pre-training. Contriever~\cite{izacard2022unsupervised} pre-train DR models on crawled large-scale web pages with Inverse Cloze Task (ICT) and Independent cropping task. COCO-DR~\cite{yu2022coco} continues to use SCL on target domain
for pre-training and leverages implicit DRO during fine-tuning to improve model robustness.
Besides, other methods to improve zero-shot DR performance include scaling up model size to increase the generalization capacity~\cite{ni2021large,kaplan2020scaling} and combining DR models with sparse retrieval methods~\cite{xu-etal-2022-laprador,chen2021salient}.


==> chapters/4_experiment.tex <==
\section{Experiment Setup}
In this section, we present our experimental settings, including datasets, baselines, and implementation details.

\subsection{Dataset and Metrics}
Following recent zero-shot DR research, we use MS MARCO Passage Ranking dataset~\cite{nguyen2016msmarco} as the source domain, with a corpus of 8.8M passages from web pages and 0.5M training queries. Each training query is coupled with a manually labeled positive passage, which together constitute the source supervised signals. We also use 43 test queries from the TREC 2019 (DL2019) as the in-domain test set for the sake of the integrity of the experiment.

As for the out-of-domain test sets, we select the BEIR dataset~\cite{thakur2021beir} and the Lotte benchmark~\cite{santhanam2021colbertv2}. BEIR is a heterogeneous evaluation benchmark for information retrieval and contains 18 datasets from diverse text retrieval tasks, from which we select publicly available datasets to conduct experiments. The Lotte benchmark consists of a collection of questions and answers sourced from the StackExchange platform, which are then divided into five distinct topics: writing, recreation, science, technology, and lifestyle. In this benchmark, the relevance of the answers is determined by their acceptance status or upvote count on the original platform. We summarize the statistics of the above datasets in Table \ref{tab:dataset}.
\begin{table*}[h]
\caption{Statistics of MSMARCO and out-of-domain datasets. The table summarizes the number of queries and documents with their average lengths. Avg. D/Q indicates the average relevant documents per query. We only select five representitive datasets from BEIR here.}
\label{tab:dataset}
\begin{tabular}{|l|l|l|lll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{Domain}} & \multicolumn{1}{c|}{Train}  & \multicolumn{3}{c|}{Test}                                                                      & \multicolumn{2}{c|}{Avg. \#Words}                          \\ \cline{3-8} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\#Pair} & \multicolumn{1}{c|}{\#Query} & \multicolumn{1}{c|}{\#Document} & \multicolumn{1}{c|}{Avg. D/Q} & \multicolumn{1}{c|}{Query} & \multicolumn{1}{c|}{Document} \\ \hline
MSMARCO                                        & Misc                                         & 532761                      & 43                           & 8841823                         & 95.4                          & 5.96                       & 55.98                         \\ \hline
TREC-COVID                                     & Bio-Medical                                  & -                           & 50                           & 171,332                         & 493.5                         & 10.60                      & 160.77                        \\
FiQA-2018                                      & Finance                                      & -                           & 648                          & 57,638                          & 2.6                           & 10.77                      & 132.32                        \\
SciFact                                        & Scientific                                   & -                           & 300                          & 5,183                           & 1.1                           & 12.37                      & 213.63                        \\
SciDocs                                        & Scientific                                   & -                           & 1,000                        & 25,657                          & 4.9                           & 9.38                       & 176.19                        \\
Touche2020                                     & Misc                                         & -                           & 49                           & 382,545                         & 19.0                          & 6.55                       & 292.37                        \\ \hline
Lotte-Wri                                      & Writing                                      & -                           & 2,000                        & 199,994                         & 6.45                          & 9.56                       & 120.45                        \\
Lotte-Life                                     & Lifestyle                                    & -                           & 2,002                        & 119,461                         & 5.13                          & 11.13                      & 152.77                        \\
Lotte-Rec                                      & Recreation                                   & -                           & 2,002                        & 166,975                         & 3.47                          & 9.58                       & 137.67                        \\
Lotte-Sci                                      & Science                                      & -                           & 2,017                        & 1,694,164                       & 7.69                          & 9.10                       & 127.74                        \\
Lotte-Tech                                     & Technology                                   & -                           & 2,004                        & 638,509                         & 7.93                          & 9.66                       & 144.95                        \\ \hline
\end{tabular}
\end{table*}

To measure the retrieval performance of DR models, we use NDCG@10 as the evaluation metrics. We also report Recall@100, Recall@1000 to reflect the retrieval capacity over the entire search corpus.

\subsection{Baselines}
We consider various baselines, including standard sparse and dense retrieval models. For sparse models, we select BM25\cite{bm25robertson1994some} as representative.
For dense models, we consider the following three types of baselines.

\textbf{Dense retrieval methods}: The models of this type are standard dual-encoder structures. DPR is trained using bm25 and in-batch negatives, while ANCE~\cite{xiong2020approximateANCE} is trained using hard negatives retrieved from the previous epoch. TAS-B~\cite{hofstatter2021efficiently} employs knowledge distillation to improve the retrieval performance. Although it is not fair to compare ANCE and TAS-B with our method since we don't employ sophisticated training strategies, we still report the results for reference.

% \textbf{Late-interaction methods}: We include ColBERT~\cite{khattab2020colbert}, which employs multiple contextualized embeddings for each token of queries
% and documents and leverages the MaxSim function to retrieve relevant documents. ColBERT has a significant advantage over the standard single-vector representation models in terms of retrieval performance, but also has a larger storage overhead and higher query latency. 

\textbf{Domain adaption methods}: We also compare RMSC with a variety of domain adaption methods. MoDIR~\cite{xin-etal-2022-modir} utilizes a momentum-based updating method with adversarial learning for domain adaptation. 
Contriever~\cite{izacard2022unsupervised} pre-trains DR models on crawled large-scale web pages with Inverse Cloze Task (ICT) and Independent cropping task. 
Condenser~\cite{gao2021condenser} enforces the [CLS] token to be the information bottleneck to aggregate attention over the entire input texts during pre-training. Thereby, the DR model can better capture the semantic information using the representation of the [CLS] token.
On top of Condenser, coCondenser~\cite{gao2021unsupervised} additionally employs the SCL task for pre-training, which significantly improves the retrieval performance.
COCO-DR~\cite{yu2022coco} continues to use SCL on target domain for pre-training  to alleviate the distribution shift, while employing implicit DRO during fine-tuning to improve model robustness.

\textbf{Query generation methods}:
QGen~\cite{ma-etal-2021-qgen} uses a T5-based query generation model, which is fine-tuned on MS MARCO, to generate 5 queries for each document in the target corpus as additional training data. A well-tuned DR model is then fine-tuned on the generated data for domain adaptation.
Following QGen, GPL~\cite{wang-etal-2022-gpl} first generates queries for documents in the target corpus, and then leverages an additional cross-encoder to score the generated query-document pairs as pseudo labels for efficient denoising, which enables training with mined hard negatives.

\subsection{Implementation Details}
We build our models based on PyTorch Framework and HuggingFace Library. When implementing RMSC, the number of special tokens $k$ is set to 1, and each special token is randomly initialized. For weak supervision extraction, we use the NLTK library to divide a document into sentences. In addition, for documents with titles, we treat the title as a sentence as well. As for the training settings of RMSC, we adopt random negative sampling and select one negative document for each query. The ICT method is used for weak supervision extraction for the Lotte dataset and SCL for the BEIR dataset. We use AdamW optimizer during training. The batch size is set to 512 and the learning rate is set to 1e-5.
We use the same random negative sampling strategy to fine-tune Condenser, coCondenser and COCO-DR for fair comparison.
At inference time, we use the Faiss ANN Library~\cite{johnson2019billionFaiss} to build index for efficient retrieval over the entire search corpus.\footnote{We will release all
the source code and trained model checkpoints upon acceptance.}





==> chapters/5_experiment_result.tex <==
\section{Experiments}

Now we empirically evaluate the proposed RMSC to address the following three research questions:
\begin{itemize}
\item \textbf{RQ1}: Can RMSC substantially improve the retrieval performance over DR models in the target domain?
\item \textbf{RQ2}: How does RMSC perform compared with other domain adaptation methods? 
\item \textbf{RQ3}: Is RMSC stable during training and is RMSC scale with other methods?

\end{itemize}
\subsection{Main Results on Lotte}
This section compares our model with other baselines on Lotte dataset to answer RQ1.

% Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \caption{Results of RMSC and different 
% baseline models on the Lotte dataset. RMSC is initialized with Condenser. $\flat$/$\natural$ and $\dag$/$\ddag$ indicates statistically significant results over the strongest baselines Contriever and COCO-DR with $p< 0.05/0.01$, respectively. The best results are marked bold. The second-best results are underlined.}
% \label{tab:lotte}
% \begin{tabular}{|cl|l|l|lllllll|cc|}
% \hline
% \multicolumn{1}{|l}{\multirow{2}{*}{\textbf{Datasets}}} &
%   \multirow{2}{*}{\textbf{Metrics}} &
%   \multicolumn{1}{c|}{\textbf{Sparse}} &
%   \multicolumn{1}{c|}{\textbf{Late-Int.}} &
%   \multicolumn{7}{c|}{\textbf{Dense}} &
%   \multicolumn{2}{c|}{\textbf{Ours}} \\ \cline{3-13} 
% \multicolumn{1}{|l}{} &
%    &
%   \multicolumn{1}{c|}{BM25} &
%   \multicolumn{1}{c|}{ColBERT} &
%   \multicolumn{1}{c}{DPR} &
%   \multicolumn{1}{c}{ANCE} &
%   \multicolumn{1}{c}{TAS-B} &
%   \multicolumn{1}{c}{Cond} &
%   \multicolumn{1}{c}{coCon} &
%   \multicolumn{1}{c}{Contr.} &
%   \multicolumn{1}{c|}{COCO} &
%   \multicolumn{1}{c}{RMSC(CD)} &
%   \multicolumn{1}{c|}{RMSC(CO)} \\ \hline
% \multirow{3}{*}{Lotte-Wri} &
%   N@10 &
%   0.352 &
%   0.435 &
%   0.357 &
%   0.388 &
%   0.346 &
%   0.373 &
%   0.418 &
%   0.424 &
%   0.422 &
%   \textbf{0.478}^{\ddag \natural} &
%   \underline{0.474}^{\ddag \natural} \\
%  &
%   R@100 &
%   0.541 &
%   0.618 &
%   0.547 &
%   0.573 &
%   0.564 &
%   0.593 &
%   0.645 &
%   0.639 &
%   0.656 &
%   \underline{0.723}^{\ddag \natural} &
%   \textbf{0.732}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.681 &
%   0.750 &
%   0.705 &
%   0.704 &
%   0.712 &
%   0.741 &
%   0.784 &
%   0.777 &
%   0.806 &
%   $\underline{0.866}^{\ddag \natural}$ &
%   $\textbf{0.871}^{\ddag \natural}$ \\ \hline
% \multirow{3}{*}{Lotte-Life} &
%   N@10 &
%   0.305 &
%   0.421 &
%   0.385 &
%   0.423 &
%   0.406 &
%   0.384 &
%   0.440 &
%   0.459 &
%   0.427 &
%   \underline{0.463}^\ddag &
%   \textbf{0.470}^{\ddag \flat} \\
%  &
%   R@100 &
%   0.548 &
%   0.677 &
%   0.648 &
%   0.680 &
%   0.686 &
%   0.668 &
%   0.737 &
%   0.746 &
%   0.718 &
%   \underline{0.784}^{\ddag \natural} &
%   \textbf{0.794}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.754 &
%   0.851 &
%   0.848 &
%   0.855 &
%   0.872 &
%   0.861 &
%   0.908 &
%   0.907 &
%   0.895 &
%   \underline{0.939}^{\ddag \natural} &
%   \textbf{0.946}^{\ddag \natural} \\ \hline
% \multirow{3}{*}{Lotte-Rec} &
%   N@10 &
%   0.325 &
%   0.427 &
%   0.362 &
%   0.403 &
%   0.390 &
%   0.376 &
%   0.431 &
%   0.443 &
%   0.424 &
%   \underline{0.462}^{\ddag \natural} &
%   \textbf{0.475}^{\ddag \natural} \\
%  &
%   R@100 &
%   0.570 &
%   0.671 &
%   0.598 &
%   0.629 &
%   0.651 &
%   0.629 &
%   0.711 &
%   0.709 &
%   0.689 &
%   \underline{0.764}^{\ddag \natural} &
%   \textbf{0.778}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.736 &
%   0.816 &
%   0.770 &
%   0.775 &
%   0.811 &
%   0.801 &
%   0.867 &
%   0.857 &
%   0.849 &
%   \underline{0.903}^{\ddag \natural} &
%   \textbf{0.906}^{\ddag \natural} \\ \hline
% \multirow{3}{*}{Lotte-Sci} &
%   N@10 &
%   0.156 &
%   \textbf{0.180} &
%   0.131 &
%   0.149 &
%   0.133 &
%   0.123 &
%   0.134 &
%   0.158 &
%   0.159 &
%   0.157 &
%   \underline{0.176}^{\ddag \natural} \\
%  &
%   R@100 &
%   0.303 &
%   0.320 &
%   0.249 &
%   0.282 &
%   0.281 &
%   0.252 &
%   0.272 &
%   0.304 &
%   0.326 &
%   \underline{0.346}^{\ddag \natural} &
%   \textbf{0.379}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.498 &
%   0.485 &
%   0.418 &
%   0.453 &
%   0.463 &
%   0.427 &
%   0.448 &
%   0.497 &
%   0.556 &
%   \underline{0.578}^{\ddag \natural} &
%   \textbf{0.632}^{\ddag \natural} \\ \hline
% \multirow{3}{*}{Lotte-Tech} &
%   N@10 &
%   0.151 &
%   0.197 &
%   0.155 &
%   0.188 &
%   0.167 &
%   0.157 &
%   0.200 &
%   0.199 &
%   0.205 &
%   \underline{0.220}^{\dag \flat} &
%   \textbf{0.234}^{\ddag \natural} \\
%  &
%   R@100 &
%   0.335 &
%   0.391 &
%   0.318 &
%   0.367 &
%   0.360 &
%   0.345 &
%   0.430 &
%   0.415 &
%   0.445 &
%   \underline{0.491}^{\ddag \natural} &
%   \textbf{0.526}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.539 &
%   0.600 &
%   0.524 &
%   0.576 &
%   0.595 &
%   0.567 &
%   0.669 &
%   0.660 &
%   0.708 &
%   \underline{0.753}^{\ddag \natural} &
%   \textbf{0.787}^{\ddag \natural} \\ \hline
% \multirow{3}{*}{Avg} &
%   N@10 &
%   0.258 &
%   0.332 &
%   0.278 &
%   0.310 &
%   0.288 &
%   0.282 &
%   0.324 &
%   0.336 &
%   0.327 &
%   \underline{0.355}^{\ddag \natural} &
%   \textbf{0.366}^{\ddag \natural} \\
%  &
%   R@100 &
%   0.459 &
%   0.535 &
%   0.472 &
%   0.506 &
%   0.508 &
%   0.497 &
%   0.565 &
%   0.562 &
%   0.566 &
%   \underline{0.621}^{\ddag \natural} &
%   \textbf{0.642}^{\ddag \natural} \\
%  &
%   R@1000 &
%   0.641 &
%   0.700 &
%   0.653 &
%   0.672 &
%   0.690 &
%   0.679 &
%   0.735 &
%   0.739 &
%   0.762 &
%   \underline{0.807}^{\ddag \natural} &
%   \textbf{0.828}^{\ddag \natural} \\ \hline
% \end{tabular}
% \end{table*}


\begin{table*}[]
\caption{Results of RMSC and different 
baseline models on the Lotte dataset. $\flat$/$\natural$ and $\dag$/$\ddag$ indicates statistically significant results over the strongest baselines Contriever and COCO-DR with $p< 0.05/0.01$, respectively. The best results are marked bold. The second-best results are underlined.}
\label{tab:lotte}
\begin{tabular}{|cl|l|lllllll|cc|}
\hline
\multicolumn{1}{|l}{\multirow{2}{*}{\textbf{Datasets}}} &
  \multirow{2}{*}{\textbf{Metrics}} &
  \multicolumn{1}{c|}{\textbf{Sparse}} &
  % \multicolumn{1}{c|}{\textbf{Late-Int.}} &
  \multicolumn{7}{c|}{\textbf{Dense}} &
  \multicolumn{2}{c|}{\textbf{Ours}} \\ \cline{3-12} 
\multicolumn{1}{|l}{} &
   &
  \multicolumn{1}{c|}{BM25} &
  % \multicolumn{1}{c|}{ColBERT} &
  \multicolumn{1}{c}{DPR} &
  \multicolumn{1}{c}{ANCE} &
  \multicolumn{1}{c}{TAS-B} &
  \multicolumn{1}{c}{Cond} &
  \multicolumn{1}{c}{coCon} &
  \multicolumn{1}{c}{Contr.} &
  \multicolumn{1}{c|}{COCO} &
  \multicolumn{1}{c}{RMSC(CD)} &
  \multicolumn{1}{c|}{RMSC(CO)} \\ \hline
\multirow{3}{*}{Lotte-Wri} &
  N@10 &
  0.352 &
  % 0.435 &
  0.357 &
  0.388 &
  0.346 &
  0.373 &
  0.418 &
  0.424 &
  0.422 &
  \textbf{0.478}^{\ddag \natural} &
  \underline{0.474}^{\ddag \natural} \\
 &
  R@100 &
  0.541 &
  % 0.618 &
  0.547 &
  0.573 &
  0.564 &
  0.593 &
  0.645 &
  0.639 &
  0.656 &
  \underline{0.723}^{\ddag \natural} &
  \textbf{0.732}^{\ddag \natural} \\
 &
  R@1000 &
  0.681 &
  % 0.750 &
  0.705 &
  0.704 &
  0.712 &
  0.741 &
  0.784 &
  0.777 &
  0.806 &
  $\underline{0.866}^{\ddag \natural}$ &
  $\textbf{0.871}^{\ddag \natural}$ \\ \hline
\multirow{3}{*}{Lotte-Life} &
  N@10 &
  0.305 &
  % 0.421 &
  0.385 &
  0.423 &
  0.406 &
  0.384 &
  0.440 &
  0.459 &
  0.427 &
  \underline{0.463}^\ddag &
  \textbf{0.470}^{\ddag \flat} \\
 &
  R@100 &
  0.548 &
  % 0.677 &
  0.648 &
  0.680 &
  0.686 &
  0.668 &
  0.737 &
  0.746 &
  0.718 &
  \underline{0.784}^{\ddag \natural} &
  \textbf{0.794}^{\ddag \natural} \\
 &
  R@1000 &
  0.754 &
  % 0.851 &
  0.848 &
  0.855 &
  0.872 &
  0.861 &
  0.908 &
  0.907 &
  0.895 &
  \underline{0.939}^{\ddag \natural} &
  \textbf{0.946}^{\ddag \natural} \\ \hline
\multirow{3}{*}{Lotte-Rec} &
  N@10 &
  0.325 &
  % 0.427 &
  0.362 &
  0.403 &
  0.390 &
  0.376 &
  0.431 &
  0.443 &
  0.424 &
  \underline{0.462}^{\ddag \natural} &
  \textbf{0.475}^{\ddag \natural} \\
 &
  R@100 &
  0.570 &
  % 0.671 &
  0.598 &
  0.629 &
  0.651 &
  0.629 &
  0.711 &
  0.709 &
  0.689 &
  \underline{0.764}^{\ddag \natural} &
  \textbf{0.778}^{\ddag \natural} \\
 &
  R@1000 &
  0.736 &
  % 0.816 &
  0.770 &
  0.775 &
  0.811 &
  0.801 &
  0.867 &
  0.857 &
  0.849 &
  \underline{0.903}^{\ddag \natural} &
  \textbf{0.906}^{\ddag \natural} \\ \hline
\multirow{3}{*}{Lotte-Sci} &
  N@10 &
  0.156 &
  % \textbf{0.180} &
  0.131 &
  0.149 &
  0.133 &
  0.123 &
  0.134 &
  0.158 &
  \underline{0.159} &
  0.157 &
  \textbf{0.176}^{\ddag \natural} \\
 &
  R@100 &
  0.303 &
  % 0.320 &
  0.249 &
  0.282 &
  0.281 &
  0.252 &
  0.272 &
  0.304 &
  0.326 &
  \underline{0.346}^{\ddag \natural} &
  \textbf{0.379}^{\ddag \natural} \\
 &
  R@1000 &
  0.498 &
  % 0.485 &
  0.418 &
  0.453 &
  0.463 &
  0.427 &
  0.448 &
  0.497 &
  0.556 &
  \underline{0.578}^{\ddag \natural} &
  \textbf{0.632}^{\ddag \natural} \\ \hline
\multirow{3}{*}{Lotte-Tech} &
  N@10 &
  0.151 &
  % 0.197 &
  0.155 &
  0.188 &
  0.167 &
  0.157 &
  0.200 &
  0.199 &
  0.205 &
  \underline{0.220}^{\dag \flat} &
  \textbf{0.234}^{\ddag \natural} \\
 &
  R@100 &
  0.335 &
  % 0.391 &
  0.318 &
  0.367 &
  0.360 &
  0.345 &
  0.430 &
  0.415 &
  0.445 &
  \underline{0.491}^{\ddag \natural} &
  \textbf{0.526}^{\ddag \natural} \\
 &
  R@1000 &
  0.539 &
  % 0.600 &
  0.524 &
  0.576 &
  0.595 &
  0.567 &
  0.669 &
  0.660 &
  0.708 &
  \underline{0.753}^{\ddag \natural} &
  \textbf{0.787}^{\ddag \natural} \\ \hline
\multirow{3}{*}{Avg} &
  N@10 &
  0.258 &
  % 0.332 &
  0.278 &
  0.310 &
  0.288 &
  0.282 &
  0.324 &
  0.336 &
  0.327 &
  \underline{0.355}^{\ddag \natural} &
  \textbf{0.366}^{\ddag \natural} \\
 &
  R@100 &
  0.459 &
  % 0.535 &
  0.472 &
  0.506 &
  0.508 &
  0.497 &
  0.565 &
  0.562 &
  0.566 &
  \underline{0.621}^{\ddag \natural} &
  \textbf{0.642}^{\ddag \natural} \\
 &
  R@1000 &
  0.641 &
  % 0.700 &
  0.653 &
  0.672 &
  0.690 &
  0.679 &
  0.735 &
  0.739 &
  0.762 &
  \underline{0.807}^{\ddag \natural} &
  \textbf{0.828}^{\ddag \natural} \\ \hline
\end{tabular}
\end{table*}

We initialize RMSC with Condenser and COCO-DR, namely RMSC(CD) and RMSC(CO) respectively, and summarize the retrieval performance of different baseline models in Table \ref{tab:lotte}. Note that the pre-trained COCO-DR model is fine-tuned with random negative sampling strategy for fair comparison.
According to the results, RMSC outperforms all baseline models of BERT-base scale on the Lotte dataset, which confirms the efficacy of the proposed RMSC method. 

In general, the dense models can surpass traditional lexical matching methods such as BM25 on most datasets, except on the Lotte-Science, a dataset with a large number of queries and documents containing mathematical formulas, when the ability of lexical and exact match is key to the retrieval performance. 
% Besides, we believe that ColBERT also achieves remarkable performance on this dataset due to this factor.

Compared to DR baselines such as DPR, ANCE, TAS-B and Condenser, RMSC considerably improves the retrieval performance by a large margin, and on average boosts 14\% and 20\% over the best ANCE on NDCG@10 and Recall@1000, respectively. 
Notice that although ANCE and TAS-B employ sophisticated training strategies such as self-mined hard negatives and knowledge distillation, RMSC still outperforms them with a simple random negative sampling during training.
We attribute this to the fact that RMSC effectively utilizes the weak supervision extracted from the target domain to enhance the alignment of the embedding space.
Meanwhile, due to the relevance gap discussed above, weak supervision, to a certain extent, can be viewed as supervised signals with noise. This can also explain that RMSC improves more on the coarse-grained Recall metrics compared to NDCG@10, which requires the fine-grained top ranking ability. 
 
As for coCondenser and Contriever, which both utilize unsupervised contrastive learning, their performance is dramatically enhanced compared to other DR models. Since Contriever is pre-trained on a large amount of crawled web pages with mixed domains, its generalization ability and performance is slightly superior compared to coCondenser. Nevertheless, RMSC improves 5.6\% and 10\% over Contriever on NDCG@10 and Recall@1000, which further illustrates the benefit of introducing target domain-specific weak supervision.

As for COCO-DR, similar to Contriever, it also uses unsupervised contrastive learning, but directly on the target corpus, thus its retrieval capability is marginally stronger.
When initialized with COCO-DR, RMSC can further improve the retrieval performance and we attribute this to that the joint training methodology can effectively mitigate the overfitting problem. The improvement also indicates that RMSC can be combined with continues contrastive pre-training introduced in COCO-DR.

\subsection{Main Results on BEIR}
In order to answer RQ1 and RQ2, this section compares RMSC with other domain adaptation methods. Since most of the research on zero-shot DR and domain adaptation has used the BEIR benchmark, we report the retrieval performance of different DR baselines and a variety of domain adaptation methods on BEIR datasets in Table \ref{tab:beir}.


% \begin{table}[]
% \caption{Comparison to DR baselines and domain adaptation methods on
% the BEIR benchmark. We report NDCG@10 in the table. $\dag$/$\ddag$ indicates
% statistically significant results over the strongest baseline COCO-DR with $p<0.05/0.01$. The best results are marked bold. The second-best results are underlined.}
% \label{tab:beir}
% \small
% \begin{tabular}{|lllllll|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Model}} &
%   % \multicolumn{1}{l|}{\textbf{MARCO}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}TREC-\\ COVID\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Sci-\\ Fact\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Sci-\\ Docs\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{FiQA}} &
%   \multicolumn{1}{l|}{\textbf{Touche}} &
%   \textbf{Avg.} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Sparse Methods}} \\ \hline
% \multicolumn{1}{|l|}{BM25} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.656} &
%   \multicolumn{1}{l|}{0.575} &
%   \multicolumn{1}{l|}{0.158} &
%   \multicolumn{1}{l|}{0.236} &
%   \multicolumn{1}{l|}{\textbf{0.367}} &
%   \multicolumn{1}{l|}{0.398} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Dense Methods}} \\ \hline
% \multicolumn{1}{|l|}{DPR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.575} &
%   \multicolumn{1}{l|}{0.475} &
%   \multicolumn{1}{l|}{0.107} &
%   \multicolumn{1}{l|}{0.274} &
%   \multicolumn{1}{l|}{0.208} &
%   \multicolumn{1}{l|}{0.328} \\ \hline
% \multicolumn{1}{|l|}{ANCE} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.654} &
%   \multicolumn{1}{l|}{0.507} &
%   \multicolumn{1}{l|}{0.122} &
%   \multicolumn{1}{l|}{0.295} &
%   \multicolumn{1}{l|}{0.240} &
%   \multicolumn{1}{l|}{0.364} \\ \hline
% \multicolumn{1}{|l|}{TAS-B} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.482} &
%   \multicolumn{1}{l|}{0.640} &
%   \multicolumn{1}{l|}{0.148} &
%   \multicolumn{1}{l|}{0.300} &
%   \multicolumn{1}{l|}{0.162} &
%   \multicolumn{1}{l|}{0.346} \\ \hline
% \multicolumn{1}{|l|}{ColBERT} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.677} &
%   \multicolumn{1}{l|}{0.671} &
%   \multicolumn{1}{l|}{0.145} &
%   \multicolumn{1}{l|}{0.317} &
%   \multicolumn{1}{l|}{0.202} &
%   \multicolumn{1}{l|}{0.402} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Domain Adaptation Methods}} \\ \hline
% \multicolumn{1}{|l|}{MoDIR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.660} &
%   \multicolumn{1}{l|}{0.502} &
%   \multicolumn{1}{l|}{0.124} &
%   \multicolumn{1}{l|}{0.296} &
%   \multicolumn{1}{l|}{n.a} &
%   \multicolumn{1}{l|}{n.a} \\ \hline
% \multicolumn{7}{|l|}{\textbf{In-Domain Generated Pseudo Labels}} \\ \hline
% \multicolumn{1}{|l|}{QGen} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.619} &
%   \multicolumn{1}{l|}{0.644} &
%   \multicolumn{1}{l|}{0.143} &
%   \multicolumn{1}{l|}{0.308} &
%   \multicolumn{1}{l|}{0.182} &
%   \multicolumn{1}{l|}{0.379} \\ \hline
% \multicolumn{1}{|l|}{GPL} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.700} &
%   \multicolumn{1}{l|}{0.674} &
%   \multicolumn{1}{l|}{0.169} &
%   \multicolumn{1}{l|}{\textbf{0.344}} &
%   \multicolumn{1}{l|}{\underline{0.255}} &
%   \multicolumn{1}{l|}{0.428} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Pre-training for Domain Adapation}} \\ \hline
% \multicolumn{1}{|l|}{Condenser} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.739} &
%   \multicolumn{1}{l|}{0.583} &
%   \multicolumn{1}{l|}{0.141} &
%   \multicolumn{1}{l|}{0.256} &
%   \multicolumn{1}{l|}{0.175} &
%   \multicolumn{1}{l|}{0.379} \\ \hline
% \multicolumn{1}{|l|}{Contriever} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.611} &
%   \multicolumn{1}{l|}{0.678} &
%   \multicolumn{1}{l|}{0.163} &
%   \multicolumn{1}{l|}{\underline{0.329}} &
%   \multicolumn{1}{l|}{0.209} &
%   \multicolumn{1}{l|}{0.398} \\ \hline
% \multicolumn{1}{|l|}{COCO-DR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.743} &
%   \multicolumn{1}{l|}{\underline{0.734}} &
%   \multicolumn{1}{l|}{0.161} &
%   \multicolumn{1}{l|}{0.298} &
%   \multicolumn{1}{l|}{0.198} &
%   \multicolumn{1}{l|}{0.428} \\ \hline
% \multicolumn{1}{|l|}{COCO-DR$\star$} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{\underline{0.789}} &
%   \multicolumn{1}{l|}{0.709} &
%   \multicolumn{1}{l|}{0.160} &
%   \multicolumn{1}{l|}{0.307} &
%   \multicolumn{1}{l|}{0.238} &
%   \multicolumn{1}{l|}{0.441} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Our Methods}} \\ \hline
% \multicolumn{1}{|l|}{RMSC(CD)} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{\textbf{0.812}^\ddag} &
%   \multicolumn{1}{l|}{0.649} &
%   \multicolumn{1}{l|}{\underline{0.186}^\ddag} &
%   \multicolumn{1}{l|}{0.317^\dag} &
%   \multicolumn{1}{l|}{0.245^\ddag} &
%   \multicolumn{1}{l|}{\underline{0.442}^\dag} \\ \hline
% \multicolumn{1}{|l|}{RMSC(CO)} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.772} &
%   \multicolumn{1}{l|}{\textbf{0.743}} &
%   \multicolumn{1}{l|}{\textbf{0.192}^\ddag} &
%   \multicolumn{1}{l|}{0.325^\ddag} &
%   \multicolumn{1}{l|}{0.252^\ddag} &
%   \multicolumn{1}{l|}{\textbf{0.457}^\ddag} \\ \hline
% \end{tabular}
% \end{table}

\begin{table*}[]
\caption{Comparison to DR baselines and domain adaptation methods on
the BEIR dataset. We report NDCG@10 in the table. $\dag$/$\ddag$ indicates
statistically significant results over the strongest baseline COCO-DR with $p<0.05/0.01$. The best results are marked bold. The second-best results are underlined. We}
\label{tab:beir}
\small
\begin{tabular}{|c|l|lllllllll|cc|}
\hline
\multirow{2}{*}{\textbf{Datasets}} &
  \multicolumn{1}{c|}{\textbf{Sparse}} &
  \multicolumn{9}{c|}{\textbf{Dense}} &
  \multicolumn{2}{c|}{\textbf{Ours}} \\ \cline{2-13} 
 &
  \multicolumn{1}{l|}{BM25} &
  DPR &
  ANCE &
  TAS-B &
  MoDIR &
  GenQ &
  GPL &
  Cond. &
  Contr. &
  COCO &
  RMSC(CD) &
  RMSC(CO) \\ \hline
\multicolumn{13}{|l|}{\textbf{BEIR Search Tasks}} \\ \hline
\textbf{TREC-COVID} &
  0.656 &
  0.575 &
  0.654 &
  0.482 &
  0.660 &
  0.619 &
  0.700 &
  0.739 &
  0.611 &
  0.743 &
  \textbf{0.812}\ddag &
  \underline{0.772} \\
\textbf{HotpotQA} &
  \underline{0.603} &
  0.371 &
  0.456 &
  0.584 &
  0.462 &
  0.534 &
  0.582 &
  0.537 &
  \textbf{0.638} &
  0.585 &
  0.455 &
  0.583 \\ 
\textbf{FiQA} &
  0.236 &
  0.274 &
  0.295 &
  0.300 &
  0.296 &
  0.308 &
  \textbf{0.344} &
  0.256 &
  \underline{0.329} &
  0.304 &
  0.317\dag &
  0.325\ddag \\
\textbf{Touche2020} &
  \textbf{0.367} &
  0.208 &
  0.240 &
  0.162 &
  n.a. &
  0.182 &
  \underline{0.255} &
  0.175 &
  0.209 &
  0.198 &
  0.245\ddag &
  0.252\ddag \\
\textbf{NFCorpus} &
  0.325 &
  0.210 &
  0.237 &
  0.319 &
  0.244 &
  0.319 &
  0.345 &
  0.274 &
  0.328 &
  \textbf{0.357} &
  0.308 &
  \underline{0.355} \\
\textbf{NQ} &
  0.329 &
  0.398 &
  0.446 &
  0.463 &
  0.442 &
  0.358 &
  0.483 &
  0.435 &
  \textbf{0.498} &
  \underline{0.479} &
  0.391 &
  0.464 \\
\textbf{DBPedia-entity} &
  0.313 &
  0.236 &
  0.281 &
  \underline{0.384} &
  0.284 &
  0.328 &
  0.384 &
  0.343 &
  \textbf{0.413} &
  0.380 &
  0.340 &
  0.377 \\ \hline
\multicolumn{13}{|l|}{\textbf{BEIR Semantic Relatedness Tasks}} \\ \hline
\textbf{SciFact} &
  0.575 &
  0.475 &
  0.507 &
  0.640 &
  0.502 &
  0.644 &
  0.674 &
  0.583 &
  0.678 &
  \underline{0.734} &
  0.649 &
  \textbf{0.742} \\
\textbf{SciDocs} &
  0.158 &
  0.107 &
  0.122 &
  0.148 &
  0.124 &
  0.143 &
  0.169 &
  0.141 &
  0.163 &
  0.161 &
  \underline{0.186}\ddag &
  \textbf{0.192}\ddag \\
\textbf{Quora} &
  0.789 &
  0.842 &
  0.852 &
  0.835 &
  0.856 &
  0.830 &
  0.836 &
  0.851 &
  \textbf{0.865} &
  \underline{0.864} &
  0.839 &
  0.859 \\
\textbf{Fever} &
  0.753 &
  0.589 &
  0.669 &
  0.700 &
  0.680 &
  0.669 &
  \textbf{0.759} &
  0.683 &
  \underline{0.758} &
  0.725 &
  0.715 &
  0.748 \\
\textbf{Climate-Fever} &
  0.213 &
  0.176 &
  0.198 &
  0.228 &
  0.206 &
  0.175 &
  0.235 &
  0.221 &
  \underline{0.237} &
  0.199 &
  \textbf{0.237}\dag &
  0.214\dag \\
\textbf{ArguAna} &
  0.414 &
  0.414 &
  0.415 &
  0.429 &
  0.418 &
  0.493 &
  \underline{0.557} &
  0.345 &
  0.446 &
  0.456 &
  0.515\ddag &
  \textbf{0.564}\ddag \\
  \hline
\textbf{Avg.} &
  0.441 &
  0.375 &
  0.413 &
  0.436 &
  n.a. &
  0.431 &
  \underline{0.486} &
  0.429 &
  0.475 &
  0.476 &
  0.462 &
  \textbf{0.497}\dag \\ \hline
\end{tabular}
\end{table*}








% \begin{table}[]
% \caption{Comparison to DR baselines and domain adaptation methods on
% the BEIR benchmark. We report NDCG@10 in the table. $\dag$/$\ddag$ indicates
% statistically significant results over the strongest baseline COCO-DR with $p<0.05/0.01$. The best results are marked bold. The second-best results are underlined.}
% \label{tab:beir}
% \small
% \begin{tabular}{|lllllll|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Model}} &
%   % \multicolumn{1}{l|}{\textbf{MARCO}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}TREC-\\ COVID\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Sci-\\ Fact\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Sci-\\ Docs\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{FiQA}} &
%   \multicolumn{1}{l|}{\textbf{Touche}} &
%   \textbf{Avg.} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Sparse Methods}} \\ \hline
% \multicolumn{1}{|l|}{BM25} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.656} &
%   \multicolumn{1}{l|}{0.575} &
%   \multicolumn{1}{l|}{0.158} &
%   \multicolumn{1}{l|}{0.236} &
%   \multicolumn{1}{l|}{\textbf{0.367}} &
%   \multicolumn{1}{l|}{0.398} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Dense Methods}} \\ \hline
% \multicolumn{1}{|l|}{DPR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.575} &
%   \multicolumn{1}{l|}{0.475} &
%   \multicolumn{1}{l|}{0.107} &
%   \multicolumn{1}{l|}{0.274} &
%   \multicolumn{1}{l|}{0.208} &
%   \multicolumn{1}{l|}{0.328} \\ \hline
% \multicolumn{1}{|l|}{ANCE} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.654} &
%   \multicolumn{1}{l|}{0.507} &
%   \multicolumn{1}{l|}{0.122} &
%   \multicolumn{1}{l|}{0.295} &
%   \multicolumn{1}{l|}{0.240} &
%   \multicolumn{1}{l|}{0.364} \\ \hline
% \multicolumn{1}{|l|}{TAS-B} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.482} &
%   \multicolumn{1}{l|}{0.640} &
%   \multicolumn{1}{l|}{0.148} &
%   \multicolumn{1}{l|}{0.300} &
%   \multicolumn{1}{l|}{0.162} &
%   \multicolumn{1}{l|}{0.346} \\ \hline
% % \multicolumn{1}{|l|}{ColBERT} &
% %   % \multicolumn{1}{l|}{} &
% %   \multicolumn{1}{l|}{0.677} &
% %   \multicolumn{1}{l|}{0.671} &
% %   \multicolumn{1}{l|}{0.145} &
% %   \multicolumn{1}{l|}{0.317} &
% %   \multicolumn{1}{l|}{0.202} &
% %   \multicolumn{1}{l|}{0.402} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Domain Adaptation Methods}} \\ \hline
% \multicolumn{1}{|l|}{MoDIR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.660} &
%   \multicolumn{1}{l|}{0.502} &
%   \multicolumn{1}{l|}{0.124} &
%   \multicolumn{1}{l|}{0.296} &
%   \multicolumn{1}{l|}{n.a} &
%   \multicolumn{1}{l|}{n.a} \\ \hline
% \multicolumn{7}{|l|}{\textbf{In-Domain Generated Pseudo Labels}} \\ \hline
% \multicolumn{1}{|l|}{QGen} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.619} &
%   \multicolumn{1}{l|}{0.644} &
%   \multicolumn{1}{l|}{0.143} &
%   \multicolumn{1}{l|}{0.308} &
%   \multicolumn{1}{l|}{0.182} &
%   \multicolumn{1}{l|}{0.379} \\ \hline
% \multicolumn{1}{|l|}{GPL} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.700} &
%   \multicolumn{1}{l|}{0.674} &
%   \multicolumn{1}{l|}{0.169} &
%   \multicolumn{1}{l|}{\textbf{0.344}} &
%   \multicolumn{1}{l|}{\underline{0.255}} &
%   \multicolumn{1}{l|}{0.428} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Pre-training for Domain Adapation}} \\ \hline
% \multicolumn{1}{|l|}{Condenser} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.739} &
%   \multicolumn{1}{l|}{0.583} &
%   \multicolumn{1}{l|}{0.141} &
%   \multicolumn{1}{l|}{0.256} &
%   \multicolumn{1}{l|}{0.175} &
%   \multicolumn{1}{l|}{0.379} \\ \hline
% \multicolumn{1}{|l|}{Contriever} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.611} &
%   \multicolumn{1}{l|}{0.678} &
%   \multicolumn{1}{l|}{0.163} &
%   \multicolumn{1}{l|}{\underline{0.329}} &
%   \multicolumn{1}{l|}{0.209} &
%   \multicolumn{1}{l|}{0.398} \\ \hline
% \multicolumn{1}{|l|}{COCO-DR} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.743} &
%   \multicolumn{1}{l|}{\underline{0.734}} &
%   \multicolumn{1}{l|}{0.161} &
%   \multicolumn{1}{l|}{0.298} &
%   \multicolumn{1}{l|}{0.198} &
%   \multicolumn{1}{l|}{0.428} \\ \hline
% % \multicolumn{1}{|l|}{COCO-DR$\star$} &
% %   % \multicolumn{1}{l|}{} &
% %   \multicolumn{1}{l|}{\underline{0.789}} &
% %   \multicolumn{1}{l|}{0.709} &
% %   \multicolumn{1}{l|}{0.160} &
% %   \multicolumn{1}{l|}{0.307} &
% %   \multicolumn{1}{l|}{0.238} &
% %   \multicolumn{1}{l|}{0.441} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Our Methods}} \\ \hline
% \multicolumn{1}{|l|}{RMSC(CD)} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{\textbf{0.812}^\ddag} &
%   \multicolumn{1}{l|}{0.649} &
%   \multicolumn{1}{l|}{\underline{0.186}^\ddag} &
%   \multicolumn{1}{l|}{0.317^\dag} &
%   \multicolumn{1}{l|}{0.245^\ddag} &
%   \multicolumn{1}{l|}{\underline{0.442}^\dag} \\ \hline
% \multicolumn{1}{|l|}{RMSC(CO)} &
%   % \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{0.772} &
%   \multicolumn{1}{l|}{\textbf{0.743}} &
%   \multicolumn{1}{l|}{\textbf{0.192}^\ddag} &
%   \multicolumn{1}{l|}{0.325^\ddag} &
%   \multicolumn{1}{l|}{0.252^\ddag} &
%   \multicolumn{1}{l|}{\textbf{0.457}^\ddag} \\ \hline
% \end{tabular}
% \end{table}
  % We also report the original COCO-DR (COCO-DR$\star$) for reference, which is fine-tuned with self-mind hard negatives and the implicit DRO technique.
According to Table \ref{tab:beir}, RMSC outperforms all baseline models on average, which is consistent with the results on the Lotte dataset. RMSC achieves considerably retrieval performance over traditional BM25 on most out-of-domain datasets, while DR struggles.

As for domain adaptation methods, MoDIR fuses training data from different domains and leverages adversarial training
method to learn a more domain invariant representation space for
dense retrieval. RMSC also fuses data from different domains, but in a explicit way by introducing the domain tokens. QGen and GPL employ additional query generation models to generate target domain queries for training, and GPL also uses a well-trained cross-encoder re-ranking model to generate pseudo-labels. However, RMSC still substantially outperforms them without using extra generation models or cross-encoders.

Compared with retrieval-oriented pre-training baselines, RMSC has on average a 7.7\% improvement compared to Condenser and a 4.4\% improvement when initialized with COCO-DR. 
% We can also find that COCO-DR$\star$ has advantages over COCO-DR in terms of NDCG@10. We attribute this to the complex training techniques employed and we believe that these sophisticated training strategies can also be combined with RMSC, which we leave for future research.
It should be noted that the performance of COCO-DR differs from that reported in the original paper. This is due to the focus of this paper being on the impact of strong and weak supervision signals on target domain performance. As a result, we utilized random negative sampling during training instead of the iDRO and hard negative techniques used in the original COCO-DR paper, which we believe is more fair and appropriate for our research objectives.

% In addition, we observe that RMSC does not perform well on some datasets, such as NQ, HotpotQA and DBPedia. We attribute this to the fact that the corpus of these datasets is based on Wikipedia, and since all models were initially pre-trained on Wikipedia, the improvement on these datasets is very limited.

% Please refer to Table \ref{tab:beir-full} for the complete results on the BEIR dataset.





\section{Ablation Study}
In this section, we conduct an ablation study on the out-of-domain datasets to analyze the contributions of the different components in RMSC.

\subsection{Influence of Weak Supervision Extraction}
As discussed in previous sections, we explore three unsupervised methods for weak supervision extraction, namely SCL and ICT. To further study the scalability of RMSC to answer RQ3, we also employ a query generation model to generate target domain queries and treat them as weak supervision, which we denote as QGen. We use the Lotte datasets for this experiment, mainly because the test labels of each dataset in Lotte are annotated in the same way and thus remain consistent in the definition of relevance. In contrast, the tasks of different datasets in BEIR, even though they are all retrieval-related tasks, are subtly differed and the labeling criteria are not exactly the same. Therefore, we believe that the experimental results on Lotte are more stable and can accurately reflect the influence of different settings.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Ablation study of RMSC with different weak supervision extraction methods on the Lotte dataset. RMSC is initialized with Condenser and we also include the results of fine-tuned Condenser for comparison.}
\label{tab:weak}
\begin{tabular}{|c|l|c|ccc|}
\hline
\multirow{2}{*}{Datasets} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Metrics}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Condenser}} &
  \multicolumn{3}{c|}{RMSC} \\ \cline{4-6}
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{SCL} &
  \multicolumn{1}{c|}{ICT} &
  \multicolumn{1}{c|}{QGen} \\ \hline
\multirow{3}{*}{Lotte-Wri}  & N@10   & 0.373 & 0.461          & \textbf{0.478} & 0.457          \\
                            & R@100  & 0.593 & 0.717          & \textbf{0.723} & 0.675          \\
                            & R@1000 & 0.741 & 0.864          & \textbf{0.866} & 0.807          \\ \hline
\multirow{3}{*}{Lotte-Life} & N@10   & 0.384 & 0.454          & 0.462          & \textbf{0.463} \\
                            & R@100  & 0.668 & 0.776          & \textbf{0.784} & 0.764          \\
                            & R@1000 & 0.861 & \textbf{0.941} & 0.939          & 0.918          \\ \hline
\multirow{3}{*}{Lotte-Rec}  & N@10   & 0.376 & 0.446          & \textbf{0.461} & 0.442          \\
                            & R@100  & 0.629 & 0.743          & \textbf{0.757} & 0.709          \\
                            & R@1000 & 0.801 & 0.887          & \textbf{0.905} & 0.859          \\ \hline
\multirow{3}{*}{Lotte-Sci}  & N@10   & 0.123 & \textbf{0.158} & 0.157          & 0.156          \\
                            & R@100  & 0.252 & 0.344          & \textbf{0.346} & 0.321          \\
                            & R@1000 & 0.427 & 0.573          & \textbf{0.577} & 0.527          \\ \hline
\multirow{3}{*}{Lotte-Tech} & N@10   & 0.157 & 0.206          & \textbf{0.220} & 0.207          \\
                            & R@100  & 0.345 & 0.474          & \textbf{0.491} & 0.447          \\
                            & R@1000 & 0.567 & 0.742          & \textbf{0.753} & 0.689          \\ \hline
\end{tabular}
\end{table}

According to the results in Table \ref{tab:weak}, we can see that ICT generally performs better than SCL on both NDCG and Recall metrics. We believe this might be due to that the weak supervision extracted by ICT is closer to the test data in terms of query and document length distribution. 

As for QGen, it also significantly improves the out-of-domain performance compared to Condenser, suggesting that query generation techniques can be combined with RMSC. Furthermore, we find that the NDCG of QGen is comparable to ICT and SCL, while the Recall performance is significantly weaker. We argue that this is because the training data generated by query generation focuses more on the fine-grained top ranking ability, which is consistent with the previously discussed findings on the Recall performance of ANCE trained with hard negatives.

% \subsection{Influence of The Number of Special Tokens}
% RMSC introduces $K$ domain tokens and $K$ relevance tokens, we now study the influence of $K$. 

\subsection{Training Robustness}
\begin{figure}[h]
  \centering
  \includegraphics[width=1.02\linewidth]{figures/finetuning_ours.pdf}
  \caption{Performance of RMSC(CD) and RMSC(CO) over different training steps on 5 of BEIR datasets. The blue dotted line indicates the nDCG@10 on MSMARCO (in-domain) and the orange solid line indicates the performance on the corresponding BEIR dataset.}
  \label{fig:finetune-ours}
\end{figure}

In order to study the training robustness of RMSC, we plot the performance of RMSC on MSMARCO and on BEIR datasets during the training process. As we can see in Figure \ref{fig:finetune-ours}, on most datasets, the retrieval performance on
MSMARCO (in-domain) keeps improving, while the performance on BEIR (out-of-domain) maintains a steady upward trend without the instability and fluctuation during direct fine-tuning. We attribute this to that RMSC utilizes target weak data and joint training methodology, thus alleviating the overfitting to the source domain features during training, which further validates the stability and robustness of the proposed RMSC.






